Knowledge Distillation from A Stronger Teacher

Unlike existing knowledge distillation methods focus on the baseline settings, where the teacher models and training strategies are not that strong and competing as state-of-the-art approaches, this paper presents a method dubbed DIST to distill better from a stronger teacher. We empirically find that the discrepancy of predictions between the student and a stronger teacher may tend to be fairly severer. As a result, the exact match of predictions in KL divergence would disturb the training and make existing methods perform poorly. In this paper, we show that simply preserving the relations between the predictions of teacher and student would suffice, and propose a correlation-based loss to capture the intrinsic inter-class relations from the teacher explicitly. Besides, considering that different instances have different semantic similarities to each class, we also extend this relational match to the intra-class level. Our method is simple yet practical, and extensive experiments demonstrate that it adapts well to various architectures, model sizes and training strategies, and can achieve state-of-the-art performance consistently on image classification, object detection, and semantic segmentation tasks. Code is available at: https://github.com/hunto/DIST_KD .

==> others/minted_code.tex <==
\vspace{-2mm}
\begin{minted}[
frame=lines,
framesep=2mm,
xleftmargin=5mm,
xrightmargin=5mm,
fontsize=\scriptsize,
%linenos
]
{python}
import torch.nn as nn

def cosine_similarity(a, b, eps=1e-8):
    return (a * b).sum(1) / (a.norm(dim=1) * b.norm(dim=1) + eps)

def pearson_correlation(a, b, eps=1e-8):
    return cosine_similarity(a - a.mean(1).unsqueeze(1), b - b.mean(1).unsqueeze(1), eps)

def inter_class_relation(y_s, y_t):
    return 1 - pearson_correlation(y_s, y_t).mean()

def intra_class_relation(y_s, y_t):
    return inter_class_relation(y_s.transpose(0, 1), y_t.transpose(0, 1))

class DIST(nn.Module):
    def __init__(self, beta, gamma):
        super(DIST, self).__init__()
        self.beta = beta
        self.gamma = gamma

    def forward(self, z_s, z_t):
        y_s = z_s.softmax(dim=1)
        y_t = z_t.softmax(dim=1)
        inter_loss = inter_class_relation(y_s, y_t)
        intra_loss = intra_class_relation(y_s, y_t)
        kd_loss = self.beta * inter_loss + self.gamma * intra_loss
        return kd_loss
\end{minted}
\vspace{-4mm}
\makeatletter\def\@captype{figure}\makeatother
\caption{The PyTorch~\cite{paszke2019pytorch} implementation of DIST.} \label{fig:code}

==> tables/ab_relation.tex <==
\begin{table}[h]
    \centering
    \begin{minipage}[t]{0.49\textwidth}
	\renewcommand\arraystretch{1.3}
	\setlength\tabcolsep{1mm}
	\centering
	\caption{Top-1 accuracies of using inter-class and intra-class relations on ImageNet. The student and teacher models are ResNet-18 and ResNet-34, respectively.}
	\vspace{2mm}
	\label{tab:ab_logit_class}
	\footnotesize
	%\normalsize
	\begin{tabular}{c|cc|c}
	    Method & Inter-class & Intra-class & ACC (\%) \\
	    \shline
	    KD & - & - & 71.21 \\
	    DIST (KL div.) & \faTimes & \faCheck & 70.61\\
	    DIST (KL div.) & \faCheck & \faCheck & 71.62\\
	    \hline
	    DIST & \faCheck & \faTimes & 71.63 \\
	    DIST & \faTimes & \faCheck & 71.55 \\
	    DIST & \faCheck & \faCheck & \textbf{72.07} \\
	\end{tabular}
	\vspace{-4mm}
	\end{minipage}
\end{table}

==> tables/detection.tex <==
\begin{table}[ht]
	\renewcommand\arraystretch{1.3}
	\setlength\tabcolsep{0.8mm}
	\centering
	%\begin{center}
	\caption{Results on COCO validation set. T: teacher; S: student. \\ *: We implement KD using $\tau=1$ and other settings are the same as DIST.}
	\vspace{2mm}
	\label{tab:det}
	\footnotesize
	%\normalsize
	\begin{tabular}{l|cccccc}
        Method & AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$\\
        \shline
        %\multicolumn{7}{c}{Two-stage detector}\\
        %\hline
        \multicolumn{7}{c}{\textit{Two-stage detectors}}\\
        T: \scriptsize{Cascade Mask RCNN-X101} & 45.6 & 64.1 & 49.7 & 26.2 & 49.6 & 60.0\\
        S: Faster RCNN-R50 & 38.4 & 59.0 & 42.0 & 21.5 & 42.1 & 50.3\\
        KD~\cite{hinton2015distilling}$^*$ & 39.7 & 61.2 & 43.0 & 23.2 & 43.3 & 51.7\\
        \citealp{chen2017learning} & 38.7 & 59.0 & 42.1 & 22.0 & 41.9 & 51.0\\
        \citealp{wang2019distilling} & 39.1 & 59.8 & 42.8 & 22.2 & 42.9 & 51.1 \\
        \citealp{heo2019comprehensive} & 38.9 & 60.1 & 42.6 & 21.8 & 42.7 & 50.7 \\
        \citealp{zhang2020improve} & 41.5 & 62.2 & 45.1 & 23.5 & 45.0 & 55.3\\
        \citealp{shu2021channel} & 41.7 & 62.0 & 45.5 & 23.3 & 45.5 & \textbf{55.5}\\
        \rowcolor{mygray}
        DIST & 40.4 & 61.7 & 43.8 & \textbf{23.9} & 44.6 & 52.6\\
        \rowcolor{mygray}
        DIST + mimic & \textbf{41.8} & \textbf{62.4} & \textbf{45.6} & 23.4 & \textbf{46.1} & 55.0\\
        \hline
        %\multicolumn{7}{c}{One-stage detector}\\
        %\hline
        \multicolumn{7}{c}{\textit{One-stage detectors}}\\
        T: RetinaNet-X101 & 41.0 & 60.9 & 44.0 & 23.9 & 45.2 & 54.0\\
        S: RetinaNet-R50 & 37.4 & 56.7 & 39.6 & 20.0 & 40.7 & 49.7\\
        KD~\cite{hinton2015distilling}$^*$ & 37.2 & 56.5 & 39.3 & 20.4 & 40.4 & 49.5\\
        \citealp{heo2019comprehensive} & 37.8 & 58.3 & 41.1 & 21.6 & 41.2 & 48.3\\
        \citealp{zhang2020improve} & 39.6 & 58.8 & 42.1 & 22.7 & 43.3 & 52.5\\
        \citealp{shu2021channel} & \textbf{40.8} & \textbf{60.4} & \textbf{43.4} & 22.7 & \textbf{44.5} & \textbf{55.3}\\
        \rowcolor{mygray}
        DIST & 39.8 & 59.5 & 42.5 & 22.0 & 43.7 & 53.0\\
        \rowcolor{mygray}
        DIST + mimic & 40.1 & 59.4 & 43.0 & \textbf{23.2} & 44.0 & 53.6\\
        %\hline
        %\multicolumn{8}{c}{Anchor-free detector}\\
        %\hline
        %RepPoints \\
		%\Xhline{2\arrayrulewidth}
	\end{tabular}
	\vspace{-4mm}
	%\end{center}
\end{table}


==> tables/res18.tex <==
\begin{table}[ht]
	\renewcommand\arraystretch{1.3}
	\setlength\tabcolsep{1.2mm}
	\centering
	%\begin{center}
	\caption{Evaluation results of student network ResNet-18 on ImageNet validation set. We use ResNet-34 released by Torchvision~\cite{marcel2010torchvision} as our teacher network, and follow the standard training strategy in CRD~\cite{tian2019contrastive}. We compare our DIST with CCKD~\cite{peng2019correlation}, Online KD~\cite{lan2018knowledge}, SP~\cite{tung2019similarity}, KD~\cite{hinton2015distilling}, CRD~\cite{tian2019contrastive}, SSKD~\cite{xu2020knowledge}, and DGKD~\cite{son2021densely} .$^*$: reported by CRD. $^\dag$: trained with 160 epochs.}
	\vspace{2mm}
	\label{tab:res18}
	\footnotesize
	%\normalsize
	\begin{tabular}{l|cc|c}
		\Xhline{2\arrayrulewidth}
		\multirow{2}*{Method} & Top-1 & Top-5 & \multirow{2}*{Additional costs}\\
		~ & (\%) & (\%) & \\
		\hline
		Teacher & 73.31 & 91.42 & - \\
		Student & 69.76 & 89.08 & -\\
		\hline
		CC$^*$& 69.96 & 89.17 & -\\
		Online KD & 70.55 & 89.59 & extra 2 branches of networks\\ 
		SP & 70.62 & 89.80 & - \\
		KD$^*$ & 70.66 & 89.88 & -\\
		CRD & 71.17 & 90.13 & extra 260M FLOPs\\
		SSKD & 71.62 & 90.67 & extra training stage of teacher\\
		ReviewKD & 71.61 & 90.51 & extra auxiliary layers\\
		DGKD$^\dagger$ & 71.73 & 90.82 & extra ResNet-26 assistant network \\
		\hline
		DIST & \textbf{72.07} & 90.42 & -\\
		\Xhline{2\arrayrulewidth}
	\end{tabular}
	%\vspace{-2mm}
	%\end{center}
\end{table}

==> tables/segmentation.tex <==
\begin{table}[ht]
	\renewcommand\arraystretch{1.3}
	\setlength\tabcolsep{3mm}
	\centering
	%\begin{center}
	\caption{Results on Cityscapes dataset. $*$: Our implementation.}
	\vspace{2mm}
	\label{tab:seg}
	\footnotesize
	%\normalsize
	\begin{tabular}{l|c}
        Method & mIoU (\%)\\
        \shline
        T: PSPNet-R101 & 78.55\\
        \hline
        S: PSPNet-R18 (ImageNet pretrained) & 70.09\\
        SKDS~\cite{liu2019structured} & 72.70\\
        SKDD~\cite{liu2020structured} & 74.08\\
        IFVD~\cite{wang2020intra} & 74.54\\
        CWD~\cite{shu2021channel}$^*$ & 75.54\\
        \rowcolor{mygray}
        DIST & \textbf{75.74}\\
        \hline
        S: PSPNet-R18 (train from scratch) & 63.63\\
        SKDS~\cite{liu2019structured} & 63.20\\
        SKDD~\cite{liu2020structured} & 64.68\\
        IFVD~\cite{wang2020intra} & 66.63\\
        SCKD~\cite{zhu2021student} & 67.25\\
        CWD~\cite{shu2021channel}$^*$ & 71.03\\
        \rowcolor{mygray}
        DIST & \textbf{71.78}\\
	\end{tabular}
	\vspace{-4mm}
	%\end{center}
\end{table}
